3D Equivariant Diffusion for Target-Aware Molecule Generation and Affinity Prediction

Rich data and powerful machine learning models allow us to design drugs for a specific protein target \textit{in silico}. Recently, the inclusion of 3D structures during targeted drug design shows superior performance to other target-free models as the atomic interaction in the 3D space is explicitly modeled. However, current 3D target-aware models either rely on the voxelized atom densities or the autoregressive sampling process, which are not equivariant to rotation or easily violate geometric constraints resulting in unrealistic structures. In this work, we develop a 3D equivariant diffusion model to solve the above challenges. To achieve target-aware molecule design, our method learns a joint generative process of both continuous atom coordinates and categorical atom types with a SE(3)-equivariant network. Moreover, we show that our model can serve as an unsupervised feature extractor to estimate the binding affinity under proper parameterization, which provides an effective way for drug screening. To evaluate our model, we propose a comprehensive framework to evaluate the quality of sampled molecules from different dimensions. Empirical studies show our model could generate molecules with more realistic 3D structures and better affinities towards the protein targets, and improve binding affinity ranking and prediction without retraining.

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See the Conclusion section.} 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{We will provide the complete codes and data once this paper is published. } 
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/outline.tex <==


[Introduction]


Contribution:

Target-aware equivariant diffusion model for molecular generation
Modeling both local and global constraints
Comprehensive evaluation framework
Empirical performance


greedy auto-regressive sampling will generate unrealistic fragments. 

Although other advanced sampling approaches like beam search can be applied, it will be very computational expensive for auto-regressive models in 3D space.

-->
We propose two approaches to generate molecules in 3D with a non-autoregressive graph-to-graph fashion. 

We do not voxelize the 3D space. 



% APPENDIX

- Implementation Details
(JQ)

- Proof of Equivariance
(JQ)

- Experiments for scaling effect
(WWQ)

==> tables/ring_size_w.tex <==
% \renewcommand{\arraystretch}{2}
\begin{tabular}{c|ccccccc}

\toprule
% \diagbox{Model}{Ring Size} & 3 & 4 & 5 & 6 & 7 & 8 & 9 \\
{Ring Size} & 3 & 4 & 5 & 6 & 7 & 8 & 9 \\
\midrule
Reference  & 1.7\%  & 0.0\%  & 30.2\% & 67.4\% & 0.7\%  & 0.0\% & 0.0\% \\
liGAN      & 28.1\% & 15.7\% & 29.8\% & 22.7\% & 2.6\%  & 0.8\% & 0.3\% \\
AR         & 29.9\% & 0.0\%  & 16.0\% & 51.2\% & 1.7\%  & 0.7\% & 0.5\% \\
TargetDiff & 0.0\%  & 2.8\%  & 30.8\% & 50.7\% & 12.1\% & 2.7\% & 0.9\% \\
\bottomrule
\end{tabular}
% \renewcommand{\arraystretch}{1}



==> tables/suppl_properties.tex <==
\renewcommand{\arraystretch}{1.8}
\begin{tabular}{c|cc|cc|cc|cc}
\toprule
\diagbox{Model}{Metric} & \multicolumn{2}{c|}{High Affinity ($\uparrow$)} & \multicolumn{2}{c|}{QED ($\uparrow$)}   & \multicolumn{2}{c|}{SA ($\uparrow$)} & \multicolumn{2}{c}{Diversity ($\uparrow$)} \\
 & Avg. & Med. & Avg. & Med. & Avg. & Med. & Avg. & Med.  \\
\midrule
GraphBP       & 14.2\% & 6.7\% & 0.43 & 0.45 & 0.49 & 0.48 & 0.79 & 0.78 \\
Pocket2Mol  & 49.8\% & 52.0\% & 0.56 & 0.57 & 0.74 & 0.75 & 0.69 & 0.71 \\
TargetDiff  & 51.3\% & 50.0\% & 0.48 & 0.48 & 0.58 & 0.58 & 0.72 & 0.71 \\
Reference   & -      & -      & 0.48 & 0.47 & 0.73 & 0.74 & -    & -    \\
\bottomrule
\end{tabular}
\renewcommand{\arraystretch}{1}

